Light Clients for Lazy Blockchains

Lazy blockchains decouple consensus from transaction verification and execution to increase throughput. Although they can contain invalid transactions (e.g., double spends) as a result, these can easily be filtered out by full nodes that check if there have been previous conflicting transactions. However, creating light (SPV) clients that do not see the whole transaction history becomes a challenge: A record of a transaction on the chain does not necessarily entail transaction confirmation. In this paper, we devise a protocol that enables the creation of efficient light clients for lazy blockchains. The number of interaction rounds and the communication complexity of our protocol are logarithmic in the blockchain execution time. Our construction is based on a bisection game that traverses the Merkle tree containing the ledger of all - valid or invalid - transactions. We prove that our proof system is succinct, complete and sound, and empirically demonstrate the feasibility of our scheme.

==> analysis.tex <==
The security of the protocol
relies on the completeness and succinctness of the \coracle and the \eoracle.


\begin{definition}[State Security]
\label{def:state-security}
  An interactive Prover--Verifier protocol $(P, V)$ is \emph{state secure} with safety parameter $\nu$, if
  the state commitment $\stc$ obtained by the verifier at the end of the protocol execution at round $r$
  satisfies \emph{safety} and \emph{liveness} as defined below.

  There exists a ledger $\ledger$ such that
  $\left<\transition^*(\st_0, \ledger)\right> = \stc$, and for all rounds $r' \geq r + \nu$: $\ledger$ is a \emph{prefix} of $\ledger^\cup_{r'}$ (safety) and $\ledger^\cap_r$ is a \emph{prefix} of $\ledger$ (liveness). 

\end{definition}

The theorems for succinctness and security of the protocol are given below.
Security consists of two components: completeness and soundness.


\begin{restatable}[Succinctness]{lemma}{restateSuccinctness}
\label{thm:succinctness}
Consider a consensus and execution oracle with $f$ and $g$ communication complexity respectively.
Then, the challenge game invoked at round $r$ with sizes $\ell_1$ and $\ell_2>\ell_1$ ends in $\log(\ell_1+\alpha(u+\nu))$ rounds of communication and
has a total communication complexity of $O(\log(\ell_1))+\alpha(u+\nu)(f(r)+g(r)))$.
\end{restatable}

\begin{restatable}[Completeness]{theorem}{restateCompleteness}
\label{thm:completeness}
Suppose the consensus and execution oracles are complete and the ledger is safe.
Then, the honest responder wins the challenge game against any PPT adversarial challenger.
\end{restatable}

\begin{restatable}[Soundness]{theorem}{restateSoundness}
\label{thm:soundness}
Let $H^s$ be a collision resistant hash function.
Suppose the consensus and execution oracles are complete and sound.
Then, for all PPT adversarial responders $\mathcal{A}$, an honest challenger wins the challenge game against $\mathcal{A}$ with overwhelming probability in $\lambda$.
\end{restatable}

\begin{restatable}[Tournament Runtime]{theorem}{restateTournamentRuntime}
\label{thm:tournament-runtime}
Suppose the consensus and execution oracles are complete and sound, and have $f$ and $g$ communication complexity respectively.
Consider a tournament started at round $r$ with $n$ provers.
Given at least one honest prover, for any PPT adversary $\mathcal{A}$, the tournament ends in $2n\log(|\ledger^{\cup}_r|+\alpha(u+\nu))$ rounds of communication and has a total communication complexity of $O(2n\log(|\ledger^{\cup}_r|+\alpha(u+\nu))+2n\alpha(u+\nu)(f(r)+g(r)))$, with overwhelming probability in $\lambda$.
\end{restatable}

\begin{restatable}[Security]{theorem}{restateSecurity}
\label{thm:security}
Suppose the consensus and execution oracles are complete and sound, and have $f$ and $g$ communication complexity respectively.
Consider a tournament started at round $r$ with $n$ provers.
Given at least one honest prover, for any PPT adversary $\mathcal{A}$, the state commitment obtained by the prover at the end of the tournament satisfies State Security with overwhelming probability in $\lambda$.
\end{restatable}

Proofs of the lemmas and theorems above are given in Appendix~\ref{sec:proofs}.

